Scalable Vision-Based 3D Object Detection and Monocular Depth Estimation for Autonomous Driving

This dissertation is a multifaceted contribution to the advancement of vision-based 3D perception technologies. In the first segment, the thesis introduces structural enhancements to both monocular and stereo 3D object detection algorithms. By integrating ground-referenced geometric priors into monocular detection models, this research achieves unparalleled accuracy in benchmark evaluations for monocular 3D detection. Concurrently, the work refines stereo 3D detection paradigms by incorporating insights and inferential structures gleaned from monocular networks, thereby augmenting the operational efficiency of stereo detection systems. The second segment is devoted to data-driven strategies and their real-world applications in 3D vision detection. A novel training regimen is introduced that amalgamates datasets annotated with either 2D or 3D labels. This approach not only augments the detection models through the utilization of a substantially expanded dataset but also facilitates economical model deployment in real-world scenarios where only 2D annotations are readily available. Lastly, the dissertation presents an innovative pipeline tailored for unsupervised depth estimation in autonomous driving contexts. Extensive empirical analyses affirm the robustness and efficacy of this newly proposed pipeline. Collectively, these contributions lay a robust foundation for the widespread adoption of vision-based 3D perception technologies in autonomous driving applications.

==> mono3d_secs/pics/arch.tex <==
\begin{figure*}
    \begin{subfigure}[b]{1.0\textwidth}
        \includegraphics[{width=1.0\textwidth}]{mono3d_secs/pics/Arch.png}
        
    \end{subfigure}
    \caption{\textbf{Network inference structure of YOLOMono3D.}
    The classification branch takes the feature map from ResNet, and it outputs dense prediction on objectness scores for each category and multi-class classification scores for each 3D dimension.
    The regression branch produces dense estimation of the normalized 2D/3D bounding box parameters $[x, y, w, h, cx, cy, z, sin(\alpha), cos(\alpha)]$.
    During inference, we further perform non-max suppression, followed by hill-climbing post optimization to produce final 3D detection results.
   }
    \label{fig:architecture}
\end{figure*}

==> monodepth_secs/image_infer.tex <==
\begin{figure*}
    \centering
    \includegraphics[{width=0.9\textwidth}]{monodepth_secs/monodepth_infer-crop.pdf}
    \caption{Online inference pipeline of FSNet. Dense full-scale Depth $d_0$ is first predicted from the trained network.  The prediction will be merged with sparse VO points $d_{vo}$ to produce accurate final prediction. The 3D SLIC algorithm is used to segment the image and limit the scale of the post-optimization problem. Only processes within the yellow frame needs to be trained in the training phase.
    }
    \label{fig:monodepth_infer}
\end{figure*}

==> monodepth_secs/image_init.tex <==
%\begin{figure}
%    \centering
%    \includegraphics[{width=0.35\textwidth}]{monodepth_secs/monodepth_init_range-crop.pdf}
%    \caption{Using the trained model as the reference, we demonstrate the area with reconstruction error less than 1 pixel. when the initial depth is 15 meters (upper) and 100 meters (lower). These fraction of pixels produce correct gradients at initialization.
    }
%    \label{fig:monodepth_init}
%\end{figure}

==> monodepth_secs/supsec-0-prove-proportion.tex <==
\section{}

==> monodepth_secs/table_kitti.tex <==

\begin{table*}[]
\caption{Performance of full-scale MonoDepth on KITTI Eigen Split. For scale factor, "GT" is using LiDAR median scaling methods and "None" means we directly evaluate the error without post-processing scale. "\textbf{*}" indicates methods using sequential images in test time. }
    \label{tab:kitti_test}
    \centering
    \begin{tabular*}{0.91\textwidth}{|l|c|c|c|c|c|c|c|c|}
    \hline {\bf Methods} & {\bf Scale Fac.} &  \cellcolor{red!25}{Abs Rel$\downarrow$} & \cellcolor{red!25}{Sq Rel$\downarrow$} & \cellcolor{red!25}{\bf RMSE$\downarrow$} & \cellcolor{red!25}{RMSE log$\downarrow$} & \cellcolor{blue!25}{$\delta<1.25$ $\uparrow$} & \cellcolor{blue!25}{$\delta<1.25^2$ $\uparrow$} & \cellcolor{blue!25}{$\delta<1.25^3$ $\uparrow$} \\ 
    \hline
    MonoDepth \cite{monodepth2} & GT  &   0.116  &   0.903  &   4.863  &   0.193  &   0.877  &   0.959  &   0.981  \\
     DNet \cite{xue2020toward} &  GT &  0.113  &   0.864  &   4.812  &   0.191  &   0.877  &   0.960  &   0.981  \\
    % MultiChannel (FSNet) & GT &  0.117  &   0.895  &   4.762  &   0.191  &   0.872  &   0.959  &   0.982  \\
    %  + Optical Flow (FSNet) &  GT & 0.117  &   0.881  &   4.746  &   0.191  &   0.873  &   0.959  &   0.981  \\
     \textbf{FSNet (single frame)} & GT  &   \textbf{0.113}  &   \textbf{0.857}  &   \textbf{4.623}  &   \textbf{0.189}  &   \textbf{0.876} &   \textbf{0.960}  &   \textbf{0.982}  \\
      \textbf{*FSNet (post-opt)}  & GT  & \textbf{0.111}  &   \textbf{0.829}  &   \textbf{4.393}  &   \textbf{0.185}  &   \textbf{0.883}  &   \textbf{0.961}  &   \textbf{0.983}  \\
    \hline
     DNet \cite{xue2020toward} & None &  0.118  &   0.925  &   4.918  &   0.199  &   0.862  &   0.953  &   0.979 \\
    % MultiChannel (FSNet) & None &   0.123  &   0.936  &   4.910  &   0.202  &   0.857  &   0.954  &   0.980  \\
    %+ Optical Flow (FSNet) &  None &  0.118  &   0.924  &   4.861  &   0.200  &   0.860  &   0.955  &   0.980  \\
       \textbf{FSNet (single frame)} &  None  & \textbf{0.116}  &   \textbf{0.923}  &   \textbf{4.694}  &   \textbf{0.194}  &   \textbf{0.871}  &   \textbf{0.958}  &   \textbf{0.981}  \\
       \textbf{*FSNet (post-opt)}   & None  & \textbf{0.109}  &   \textbf{0.866}  &   \textbf{4.450}  &   \textbf{0.189}  &   \textbf{0.879}  &   \textbf{0.959}  &   \textbf{0.982}  \\
      \hline
    \end{tabular*}
    
\end{table*}

==> scaleup_secs/image_infer.tex <==
\begin{figure*}
    \centering
    \includegraphics[{width=0.8\textwidth}]{secs/monodepth_infer-crop.pdf}
    \caption{Online inference pipeline of FSNet. Dense full-scale Depth $d_0$ is first predicted from the trained network.  The prediction will be merged with sparse VO points $d_{vo}$ to produce accurate final prediction. The 3D SLIC algorithm is used to segment the image and limit the scale of the post-optimization problem. Only processes within the yellow frame needs to be trained in the training phase.
    }
    \label{fig:monodepth_infer}
\end{figure*}

==> scaleup_secs/image_init.tex <==
%\begin{figure}
%    \centering
%    \includegraphics[{width=0.35\textwidth}]{secs/monodepth_init_range-crop.pdf}
%    \caption{Using the trained model as the reference, we demonstrate the area with reconstruction error less than 1 pixel. when the initial depth is 15 meters (upper) and 100 meters (lower). These fraction of pixels produce correct gradients at initialization.
    }
%    \label{fig:monodepth_init}
%\end{figure}

==> scaleup_secs/image_struct.tex <==
\begin{figure*}
    \centering
    \includegraphics[{width=0.8\textwidth}]{scaleup_secs/monodepth_struct_flow-crop.pdf}
    \caption{The training process of FSNet. Both the teacher network $\Theta_{teacher}$ and the student network $\Theta_{student}$ utilize a U-Net structure with a ResNet-18 backbone.
    $\Theta_{teacher}$ is fully-pretrained using only the photometric loss and is frozen during the training of the student network. $\Theta_{student}$ is trained with a summation of photometric loss and distillation loss. To form the photometric loss, we calculate the optical flow between two frames and use it to compute an extra mask to block error gradients from dynamic objects.
    }
    \label{fig:monodepth_struct}
\end{figure*}

==> scaleup_secs/supsec-0-prove-proportion.tex <==
\section{}

==> scaleup_secs/table_campus.tex <==
\begin{table}
    \centering
    \caption{2D Detection Results on Campus' Data, evaluate with $IoU_{2D} \geq 0.5$}
    \def\arraystretch{1.3}
    \begin{tabular*}{0.28\textwidth}{ |l|c|c|}
        \hline
        {\bf Methods} & {\bf Car} & {\bf Ped}   \\ \hline
        kittiMonoFlex & 55.4\% & 27.7\%  \\
        \hline
        TunedMonoFlex & 86.7\% &  81.90\%  \\
        \hline
    \end{tabular*}
    
    \label{tab:test_results_campus}
\end{table}

==> scaleup_secs/table_kitti.tex <==

\begin{table*}[]
\caption{Performance of full-scale MonoDepth on KITTI360 Fisheye. We directly evaluate the error without compensating scales. The \cellcolor{red!25}{pink} columns are error metrics, the lower the better; the \cellcolor{blue!25}{blue} columns are accuracy metrics, the higher the better.}
    \label{tab:kitti_test}
    \centering
    \begin{tabular*}{0.76\textwidth}{|l|c|c|c|c|c|c|c|}
    \hline {\bf Methods} &  \cellcolor{red!25}{\bf {Abs Rel}} & \cellcolor{red!25}{Sq Rel} & \cellcolor{red!25}{ RMSE} & \cellcolor{red!25}{RMSE LOG} & \cellcolor{blue!25}{$\delta<1.25$} & \cellcolor{blue!25}{$\delta<1.25^2$} & \cellcolor{blue!25}{$\delta<1.25^3$} \\ 
    \hline
       \textbf{FSNet (all depth)}   & \textbf{0.161}  &   \textbf{0.594}  &   \textbf{2.348}  &   \textbf{0.823}  &   \textbf{0.771}  &   \textbf{0.881}  &   \textbf{0.927}  \\
       \textbf{FSNet (within 8m)}     & \textbf{0.084}  &   \textbf{0.318}  &   \textbf{0.772}  &   \textbf{0.185}  &   \textbf{0.940}  &   \textbf{0.980}  &   \textbf{0.991}  \\
      \hline
    \end{tabular*}
    
\end{table*}

\begin{table*}[]
\caption{Performance of full-scale MonoDepth on KITTI Eigen Split. For scale factor, "GT" is using LiDAR median scaling methods and "None" means we directly evaluate the error without compensating scales. "\textbf{*}" indicates methods using sequential images in test time. The \cellcolor{red!25}{pink} columns are error metrics, the lower the better; the \cellcolor{blue!25}{blue} columns are accuracy metrics, the higher the better.}
    \label{tab:kitti_test}
    \centering
    \begin{tabular*}{0.88\textwidth}{|l|c|c|c|c|c|c|c|c|}
    \hline {\bf Methods} & {\bf Scale Factor} &  \cellcolor{red!25}{Abs Rel} & \cellcolor{red!25}{Sq Rel} & \cellcolor{red!25}{\bf RMSE} & \cellcolor{red!25}{RMSE LOG} & \cellcolor{blue!25}{$\delta<1.25$} & \cellcolor{blue!25}{$\delta<1.25^2$} & \cellcolor{blue!25}{$\delta<1.25^3$} \\ 
    \hline
    MonoDepth \cite{monodepth2} & GT  &   0.116  &   0.903  &   4.863  &   0.193  &   0.877  &   0.959  &   0.981  \\
     DNet \cite{xue2020toward} &  GT &  0.113  &   0.864  &   4.812  &   0.191  &   0.877  &   0.960  &   0.981  \\
     % ManyDepth* \cite{manydepth2021temporal} & GT & 0.098 & 0.770 & 4.459 & 0.176 & 0.800 & 0.965 & 0.983 \\
    % MultiChannel (FSNet) & GT &  0.117  &   0.895  &   4.762  &   0.191  &   0.872  &   0.959  &   0.982  \\
    %  + Optical Flow (FSNet) &  GT & 0.117  &   0.881  &   4.746  &   0.191  &   0.873  &   0.959  &   0.981  \\
     \textbf{FSNet (single frame)} & GT  &   \textbf{0.113}  &   \textbf{0.857}  &   \textbf{4.623}  &   \textbf{0.189}  &   \textbf{0.876} &   \textbf{0.960}  &   \textbf{0.982}  \\
      \textbf{*FSNet (post-opt)}  & GT  & \textbf{0.111}  &   \textbf{0.829}  &   \textbf{4.393}  &   \textbf{0.185}  &   \textbf{0.883}  &   \textbf{0.961}  &   \textbf{0.983}  \\
    \hline
     DNet \cite{xue2020toward} & None &  0.118  &   0.925  &   4.918  &   0.199  &   0.862  &   0.953  &   0.979 \\
    % MultiChannel (FSNet) & None &   0.123  &   0.936  &   4.910  &   0.202  &   0.857  &   0.954  &   0.980  \\
    %+ Optical Flow (FSNet) &  None &  0.118  &   0.924  &   4.861  &   0.200  &   0.860  &   0.955  &   0.980  \\
       \textbf{FSNet (single frame)} &  None  & \textbf{0.116}  &   \textbf{0.923}  &   \textbf{4.694}  &   \textbf{0.194}  &   \textbf{0.871}  &   \textbf{0.958}  &   \textbf{0.981}  \\
       \textbf{*FSNet (post-opt)}   & None  & \textbf{0.109}  &   \textbf{0.866}  &   \textbf{4.450}  &   \textbf{0.189}  &   \textbf{0.879}  &   \textbf{0.959}  &   \textbf{0.982}  \\
      \hline
    \end{tabular*}
    
\end{table*}





==> scaleup_secs/table_nusc_kitti_backup.tex <==
\begin{table*}[h!]
    \centering
    \caption{Object detection results on the KITTI validation set. For 3D metrics, cars are evaluated with $\text{IoU}_{3D} \geq 0.5$ and Pedestrians are evaluated with $\text{IoU}_{3D} \geq 0.25$; for 2D metrics, cars are evaluated with $\text{IoU}_{2D} \geq 0.7$ and Pedestrians are evaluated with $\text{IoU}_{2D} \geq 0.5$. }
    %\footnotesize
    \def\arraystretch{1.3}
    \begin{tabular*}{0.7\textwidth}{ |c|l|c|c|}
        \cline{1-4}
        {Method} &{\bf Methods} & {\bf Car Easy/Moderate/Hard} & {\bf Ped. Easy/Moderate/Hard}   \\ \cline{1-4}
        \multirow{2}{*}{$3D$} &NuscMonoFlex & 30.69\% / 23.88 \%/ 20.34 \% &  7.83\% / 6.66\% / 5.49\%  \\
        \cline{2-4}
        &TunedMonoFlex & 35.73\% / 24.90 \%/ 20.38 \% &  11.80\% / 8.84\% / 7.43\%  \\
        \cline{1-4}
        \multirow{2}{*}{$2D$} &NuscMonoFlex & 90.91\%/ 81.28\%/ 71.50\% &  59.04\%, 50.84\%, 43.76\%  \\
        \cline{2-4}
        &TunedMonoFlex & 95.95\%/ 90.42\%/ 80.36 \% &  62.40\%, 54.31\%, 47.61\%  \\
        \cline{1-4}
    \end{tabular*}
    
    \label{tab:test_results_on_cityscapes}
\end{table*}
